Text Matching Improves Sequential Recommendation by Reducing Popularity Biases

This paper proposes Text mAtching based SequenTial rEcommendation model (TASTE), which maps items and users in an embedding space and recommends items by matching their text representations. TASTE verbalizes items and user-item interactions using identifiers and attributes of items. To better characterize user behaviors, TASTE additionally proposes an attention sparsity method, which enables TASTE to model longer user-item interactions by reducing the self-attention computations during encoding. Our experiments show that TASTE outperforms the state-of-the-art methods on widely used sequential recommendation datasets. TASTE alleviates the cold start problem by representing long-tail items using full-text modeling and bringing the benefits of pretrained language models to recommendation systems. Our further analyses illustrate that TASTE significantly improves the recommendation accuracy by reducing the popularity bias of previous item id based recommendation models and returning more appropriate and text-relevant items to satisfy users. All codes are available at https://github.com/OpenMatch/TASTE.

==> limitation.tex <==
\section*{Limitations}
SREDR converts the sequential recommendation task to a text matching task and employs the dense retrieval architecture to retrieve items according to user-item interaction history. SREDR shows strong effectiveness on representing low-frequently interacted items by using names and attributes. However, compared with the methods that represent items with item embeddings, such text-based representation heavily relies on the information of items and may limit to model the potential relations among items beyond the text descriptions. Besides, to effectively model long user-item interactions, SREDR separates user-item interaction sequences to subsequences, which are regarded as sessions and independently encoded to make the self-attention more sparse. The sequence split method may cause different influences on the long user-item interaction modeling.

==> table/appablation.tex <==
\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ l | c | c |  c  | c  }
\hline
\multirow{2}{*}{\textbf{Settings}} & \multicolumn{4}{c}{\textbf{Toys}} \\ \cline{2-5}
& Recall@10   & Recall@20 & NDCG@10   & NDCG@20 \\\hline
T5-DPR w/o Prompt & 0.0777 & 0.1222 & 0.0369 & 0.0480  \\
\hline
T5-DPR & 0.0805& 0.1243 & 0.0375 & 0.0485  \\
+ Popular Negs & 0.0678 & 0.1065 & 0.0326 & 0.0423  \\
+ Hard Negs & 0.0878 & 0.1297 & 0.0426 & 0.0532  \\
+ Random Negs & 0.1032 & 0.1577 & 0.0488 & 0.0625  \\
\hline
w/ Longer History & \textbf{0.1056} & \textbf{0.1594}  & \textbf{0.0508} & \textbf{0.0643} \\
\hline
\end{tabular}}
\caption{Ablation Study on Toys Dataset.}
\label{tab:appablation}
\end{table}

==> table/appevaluate.tex <==
\begin{table}[t]
\begin{center}
\small

\begin{tabular}{l|c|   c   | c }
\hline 
\textbf{Dataset} & \textbf{Metrics} &  \textbf{DIF-SR}  &  \textbf{SREDR}\\ 
\hline
\multirow{4}{*}{Beauty} & HR@10 & 0.0909 & \textbf{0.1030}  \\
& HR@20  & 0.1278  & \textbf{0.1550}  \\
& MRR@10  & 0.0308 & \textbf{0.0362}  \\
& MRR@20  &0.0333  & \textbf{0.0398}  \\
\hline
\multirow{4}{*}{Sports} & HR@10 & 0.0540 & \textbf{0.0633}  \\
& HR@20  & 0.0783  & \textbf{0.0964}  \\
& MRR@10  & 0.0162 & \textbf{0.0248}  \\
& MRR@20  &0.0178  & \textbf{0.0271}  \\
\hline
\multirow{4}{*}{Toys} & HR@10 & 0.0953 & \textbf{0.1232}  \\
& HR@20  & 0.1343  & \textbf{0.1789}  \\
& MRR@10  & 0.0320 & \textbf{0.0460}  \\
& MRR@20  &0.0347  & \textbf{0.0498}  \\
\hline
\multirow{4}{*}{Yelp} & HR@10 & 0.0681 & \textbf{0.0738}  \\
& HR@20  & 0.0985  & \textbf{0.1156}  \\
& MRR@10  & \textbf{0.0331} & 0.0294  \\
& MRR@20  & \textbf{0.0351}  & 0.0322  \\
\hline
\end{tabular}
\end{center}
\caption{\label{tab:appeval} Additional Evaluations for Recommendation Effectiveness of SREDR. We use two additional evaluation metrics, Hit-Ratio and MRR, to evaluate the performance of SREDR and our main baseline model, DIF-SR~\cite{Xie2022DIF-SR}.}

\end{table}

==> table/case.tex <==
\begin{table*}[!ht]

\small

\begin{tabular}{p{0.1\linewidth}|p{0.8\linewidth}} 
\hline
%\makecell[l]{\textbf{Case1}} & \makecell{Yelp}
\multicolumn{2}{l}{\textbf{Case \#1 in Yelp}}
\tabularnewline 
\hline
\makecell[l]{History} & title: Stu’s Barrel House address: 3215 North Davidson St \textcolor[rgb]{0.7,0.3,0.3}{Charlotte NC}, title: Bernardin's Restaurant At Ratcliffe address: 435 S Tryon St, Ste 100, Ratcliffe \textcolor[rgb]{0.7,0.3,0.3}{Charlotte NC}, $...$,title: Inishmore address: 1315 East Blvd, Ste 130 \textcolor[rgb]{0.7,0.3,0.3}{Charlotte NC}, title: Capriccis True Italian address: 109 WS Main St Waxhaw NC
\tabularnewline 
\hline
\makecell[l]{Label} & \textcolor[rgb]{0.7,0.3,0.3}{title: Bao and Broth address: 1115 N Brevard St, Ste 15 Charlotte NC}
\tabularnewline 
\hline
\makecell[l]{T5-DPR}
&
\makecell[l]{\textit{1st:} title: Crossroads Coffee House address: 112 N Broome St Waxhaw NC \\ \textit{2nd:} title: Capriccis True Italian address: 109 WS Main St Waxhaw NC \\ \textit{3rd:} title: Stack's Kitchen address: 1315 N Broome St Waxhaw NC \\ \textit{4th:} title: 4th Corner Bakehouse and Coffee Co address: 205 Salem St Waxhaw NC \\ \textit{5th:} title: Emmet's Social Table address: 401 E South Main St Waxhaw NC}

\tabularnewline 
\hline
\makecell[l]{SREDR}
&
\makecell[l]{\textit{1st:} title: Flower Child- Charlotte address: 1537 Camden Rd Charlotte NC \\ \textit{2nd:} title: Eight and Sand Kitchen address: 135 New Bern St Charlotte NC \\ \textit{3rd:} \textcolor[rgb]{0.7,0.3,0.3}{title: Bao and Broth address: 1115 N Brevard St, Ste 15 Charlotte NC} \\ \textit{4th:} title: Dot Dot Dot address: 4237 Park Rd, Unit B Charlotte NC \\ \textit{5th:} title: Queen City Grounds address: 644 N Church St Charlotte NC}
\tabularnewline 
\hline
\multicolumn{2}{l}{\textbf{Case \#2 in Beauty}}
%\makecell[l]{\textbf{Case2}} & \makecell{Beauty}
\tabularnewline 
\hline
\makecell[l]{History} & title: Simple Revitalizing Eye RollOn, 0.5 Ounce, title: Sally Hansen Hard as \textcolor[rgb]{0.7,0.3,0.3}{Nails} Hard as Wraps, Clear, 0.4 Fluid Ounce, title: Simple Soothing Eye Balm, 0.5 Ounce, title: Banana Boat Summer Color Self-Tanning Mist Airbrush Color, title: Revlon Shine Enchancing Hot Air Kit, title: Garnier Skin Renew Miracle Skin Perfector B.B. Cream, title: MASH 5 X 2 Way Marbleizing Dotting Tool Pen Set for \textcolor[rgb]{0.7,0.3,0.3}{Nail} Art Manicure Pedicure
\tabularnewline 
\hline
Label & \textcolor[rgb]{0.7,0.3,0.3}{title: World Pride Nail Tape Stripe Decoration Sticker Hologram, Set of 10}
\tabularnewline 
\hline
T5-DPR
&
\makecell[l]{\textit{1st:} title: Sally Hansen Magnetic Nail Color - Ionic Indigo \\ \textit{2nd:} title: Sally Hansen Color Quick Chromes Nail Enamel \\ \textit{3rd:} title: Sally Hansen Salon Effects Real Nail Polish Strips \\ \textit{4th:} Sally Hansen Hard As Nails French Manicure Set \\ \textit{5th:} Sally Hansen Mega Shine Nail Treatment}

\tabularnewline 
\hline
SREDR
&
\makecell[l]{\textit{1st:} title: title: Nail Art Brushes- Professional Nail Art Brushes \\ \textit{2nd:} title: Dotting 5 X 2 Way Marbleizing Dotting Pen Set for Nail Art Manicure Pedicure \\ \textit{3rd:} title: 15pcs Nail Art Painting Pen Brush \\ \textit{4th:} title: MASH Rhinestones 2400 Piece 12 Color Nail Art Nailart Manicure Wheels \\ \textit{5th:} \textcolor[rgb]{0.7,0.3,0.3}{title: World Pride Nail Tape Stripe Decoration Sticker Hologram, Set of 10}}
\tabularnewline 
\hline
\multicolumn{2}{l}{\textbf{Case \#3 in Sports}}
%\textbf{Case3} & \makecell{Sports}
\tabularnewline 
\hline
History & title: Russell Athletic Men's Big Tall Basic Crew Neck Sweatshirt, title: Victorinox Swiss Army Classic SD Pocket Knife,$...$,title: SKLZ Rain Maker - Trajectory Rebounding \textcolor[rgb]{0.7,0.3,0.3}{Basketball Trainer}, title: SKLZ SpeedSac - Variable Weight Sprint \textcolor[rgb]{0.7,0.3,0.3}{Trainer}, title: SKLZ Speed Striker - Agility Cardio Boxing \textcolor[rgb]{0.7,0.3,0.3}{Trainer}, title: SKLZ Core Wheels Dynamic Strength Ab \textcolor[rgb]{0.7,0.3,0.3}{Trainer}, title: NOCO Genius G7200 12V/24V 7.2 Amp Smart Battery Charger and Maintainer
\tabularnewline 
\hline
Label & \textcolor[rgb]{0.7,0.3,0.3}{title: SKLZ ShotLoc Basketball Shooting Trainer}
\tabularnewline 
\hline
T5-DPR
&
\makecell[l]{\textit{1st:} title: Ringside Apex Boxing Gloves \\ \textit{2nd:} title: SKLZ Reaction Belts Partnered Breakaway Trainer \\ \textit{3rd:} title: Venum Kontact Gel Glove Wraps, Black \\ \textit{4th:} title: Thule Chariot Cheetah Double Stroller - Green \\ \textit{5th:} title: Venum Elite Boxing Gloves}
\tabularnewline 
\hline
SREDR
&
\makecell[l]{\textit{1st:} title: Tasc Performance Men's Carrollton Performance Running Tee Shirt \\ \textit{2nd:} title: Hydracentials Slim Grip 25oz Stainless Steel Water Bottle \\ \textit{3rd:} title: SKLZ Reaction Belts Partnered Breakaway Trainer \\ \textit{4th:} title: SKLZ Kool 'N Fit Sport Performance Spray \\ \textit{5th:} \textcolor[rgb]{0.7,0.3,0.3}{title: SKLZ ShotLoc Basketball Shooting Trainer}}

\tabularnewline 
\hline
\multicolumn{2}{l}{\textbf{Case \#4 in Toys}}
%\textbf{Case4} & \makecell{Toys}
\tabularnewline 
\hline
History & title: Melissa Doug Large Wooden See Inside ABC Puzzle, 26-Piece, title: Fisher Price Twirlin' Whirlin Garden, title: \textcolor[rgb]{0.7,0.3,0.3}{My First LeapPad} Learning System - Blue, title: \textcolor[rgb]{0.7,0.3,0.3}{Thomas} and Friends Train Play Set - Thomas Big Loader
\tabularnewline 
\hline
Label & \textcolor[rgb]{0.7,0.3,0.3}{title: LeapFrog My First LeapPad Educational Book: Thomas and the School Trip}
\tabularnewline 
\hline
T5-DPR
&
\makecell[l]{\textit{1st:} title: Thomas and Friends Train Play Set - Thomas Big Loader \\ \textit{2nd:} title: Geo Trax Working Town Railway System with exclusive bonus \\ \textit{3rd:} title: Thomas and Friends Spin Fix Thomas \\ \textit{4th:} title: Thomas And Friends Wooden Railway - Early Engineers Busy Day on Sodor Set \\ \textit{5th:} title: Tinkertoy Classic Construction Set: Junior Builder}

\tabularnewline 
\hline
SREDR
&
\makecell[l]{\textit{1st:} title: Thomas and Friends Train Play Set - Thomas Big Loader \\ \textit{2nd:} title: My First LeapPad Learning System - Blue \\ \textit{3rd:} title: LeapFrog Original LeapPad Learning System from 2004 \\ \textit{4th:} title: LeapFrog MyFirst LeapPad Learning System- Pooh's Honey Tree \\ \textit{5th:} \textcolor[rgb]{0.7,0.3,0.3}{title: LeapFrog My First LeapPad Educational Book: Thomas and the School Trip}}

\tabularnewline 
\hline 
\end{tabular}
 \caption{Case Studies. We select several cases from the four datasets, Yelp, Beauty, Sports, and Toys, to show Top-5 retrieved items from SREDR and T5-DPR.}
 \label{tab:case_study}
\end{table*}

==> table/cold.tex <==
\begin{table}[t]
\begin{center}
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l | c | c c}
\hline 
\textbf{Dataset} & \textbf{\#Total}  & \textbf{\#Low Frequency} & \textbf{\#Higher Frequency}  \\ \hline
Beauty & 2,930 & 4,802 & 17,561 \\
Yelp & 1,889 & 2,360 & 28,139 \\
Sports & 4,805 & 7,875 & 27,723 \\
Toys & 2,978 & 4,983 & 14,429 \\
\hline
\end{tabular}}
\end{center}
\caption{\label{tab:coldsplit}Item Statistics with Different User Interacted Frequencies. We split the testing datasets into two groups, low frequency and higher frequency, according to the user interacted frequency of items.}
\end{table}

==> table/completeablation.tex <==
% \begin{table*}[t]
% \centering
% % \small
% \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{ l | c| c| c  | c |c | c  | c |c |c }
% \hline
% \multirow{2}{*}{\textbf{Settings}} & \multicolumn{3}{c|}{\textbf{Yelp}} & \multicolumn{3}{c|}{\textbf{Sports}} & \multicolumn{3}{c}{\textbf{Beauty}}\\ \cline{2-10}
% & Recall@10 & NDCG@10 & NDCG@20   & Recall@10 & NDCG@10 & NDCG@20  & Recall@10 & NDCG@10 & NDCG@20 \\\hline
% T5-DPR w/o Prompt & 0.0441 & 0.0235 & 0.0304 & 0.0327 & 0.0155 & 0.0211 & 0.0688 & 0.0335 & 0.0435  \\
% \hline
% T5-DPR & 0.0460& 0.0250 & 0.0320 & 0.0329 & 0.0159 & 0.0216 & 0.0716 & 0.0345 & 0.0437  \\
% + Popular Negs & 0.0351 & 0.0186 & 0.0236 & 0.0284 & 0.0135 & 0.0184 & 0.0601 & 0.0294 & 0.0382  \\
% + Hard Negs & 0.0324 & 0.0173 & 0.0222 & 0.0354 & 0.0182 & 0.0232 & 0.0750 & 0.0368 & 0.0468  \\
% + Random Negs & 0.0726 & 0.0388 & 0.0489 & 0.0510 & 0.0249 & 0.0325 & 0.0921 & 0.0444 & 0.0565  \\
% \hline
% w/ Longer History & \textbf{0.0733} & \textbf{0.0393}  & \textbf{0.0498} & \textbf{0.0545} & \textbf{0.0270} & \textbf{0.0346} & \textbf{0.0935} &\textbf{0.0445} & \textbf{0.0573} \\
% \hline
% \end{tabular}
% }
% \caption{Ablation Study. }
% \label{tab:comablation}
% \end{table*}


\begin{table*}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c| c|  c  c   c  c  |  c  }
\hline 
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Metrics}} &  \textbf{T5-DPR w/o Prompt} &  \multicolumn{4}{c|}{\textbf{T5-DPR}} & \textbf{T5-DPR (Rand Negs)} \\
& &\textbf{(Inbatch)} & \textbf{Inbatch}  & \textbf{Popular Negs}  & \textbf{Hard Negs} & \textbf{Random Negs} & \textbf{w/ Longer History} \\ 
\hline
\multirow{4}{*}{Yelp} & Recall@10 & 0.0441 &  0.0460  &0.0351 & 0.0324 & 0.0726& \textbf{0.0733}  \\
& Recall@20  & 0.0714  & 0.0740 & 0.0550 & 0.0519 & 0.1131& \textbf{0.1150}  \\
& NDCG@10  & 0.0235 & 0.0250 & 0.0186& 0.0173 & 0.0388& \textbf{0.0393}  \\
& NDCG@20  &0.0304  & 0.0320 & 0.0236 & 0.0222 & 0.0489& \textbf{0.0498}  \\
\hline
\multirow{4}{*}{Sports} & Recall@10   &0.0327 &0.0329 & 0.0284 & 0.0354 & 0.0510& \textbf{0.0545} \\
& Recall@20 &0.0550 &0.0554 &0.0476 & 0.0550 & 0.0812& \textbf{0.0851} \\
& NDCG@10  &0.0155 &0.0159 &0.0135 & 0.0182 & 0.0249& 
 \textbf{0.0270}  \\
& NDCG@20 &0.0211 &0.0216 & 0.0184 & 0.0232 & 0.0325& \textbf{0.0346}  \\
\hline
\multirow{4}{*}{Beauty} & Recall@10  & 0.0688 & 0.0716 &  0.0601  &0.0750 & 0.0921 & \textbf{0.0935} \\
& Recall@20  & 0.1088  & 0.1082 & 0.0950 & 0.1147 & 0.1401& \textbf{0.1441} \\
& NDCG@10 & 0.0335 & 0.0345 & 0.0294  & 0.0368 & 0.0444& \textbf{0.0445} \\
& NDCG@20 &0.0435  & 0.0437 & 0.0382 & 0.0468 & 0.0565& \textbf{0.0573} \\
\hline
\multirow{4}{*}{Toys} & Recall@10  & 0.0777 &  0.0805  &0.0678  & 0.0878 & 0.1032& \textbf{0.1056} \\
& Recall@20 & 0.1222  & 0.1243 & 0.1065 & 0.1297 & 0.1577& \textbf{0.1594} \\
& NDCG@10  & 0.0369 & 0.0375 & 0.0326 & 0.0426 & 0.0488& \textbf{0.0508}  \\
& NDCG@20 &0.0480  & 0.0485 & 0.0423 & 0.0532 & 0.0625& \textbf{0.0643} \\
 \hline

\end{tabular}}
\caption{\label{tab:comablation}More Experimental Results of Ablation Study.}

\end{table*}

==> table/datastatistic.tex <==
\begin{table}[t]
\begin{center}
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l  r  r r r}
\hline \textbf{Dataset} & \textbf{Beauty} & \textbf{Yelp} & \textbf{Sports} & \textbf{Toys}\\ \hline
Users & 22,363 & 30,499 & 35,598 & 19,412   \\
Items & 12,101 & 20,068 & 18,357 & 11,924   \\
Interactions & 198,502 & 317,182 & 296,337 & 167,597   \\
Avg Item Length & 9 & 10 & 8 & 9   \\
Sparsity & 99.93\% & 99.95\% & 99.95\% & 99.93\%   \\ \hline
\end{tabular}}
\caption{\label{tab:dataset}Data Statistics of Yelp and Amazon Product. Amazon Product consists of Beauty, Sports, and Toys.}
\end{center}
\end{table}

==> table/itemverb.tex <==
\begin{table*}[!ht]

\small
\begin{tabular}{p{0.2\linewidth}|p{0.7\linewidth}} 
\hline
\multicolumn{2}{l}{\textbf{Yelp}}
\tabularnewline 
\hline
User Interaction History & Here is the visit history list of user: id: 18078 title: Freed's Bakery address: 9815 S Eastern Ave Las Vegas NV, id: 650 title: Trattoria Italia address: 9905 S Eastern Ave, Ste 140 Las Vegas NV, id: 10540 title: Starbucks address: 3410 E Sunset Road Las Vegas NV, id: 16529 title: Starbucks address: 8975 S. Eastern Avenue, Las Vegas NV recommend next item
\tabularnewline 
\hline
Next Item & id: 6084 title: El Dorado Cantina address: 3025 Sammy Davis Jr Dr Las Vegas NV
\tabularnewline 
\hline

\multicolumn{2}{l}{\textbf{Beauty}}
\tabularnewline 
\hline
User Interaction History & Here is the visit history list of user: id: 8005 title: Neutrogena Ultra Gentle Soothing Lotion SPF 15, 4  Ounce, id: 451 title: GRANDPA'S BRANDS, Pine Tar Soap Bath Size - 4.25 oz, id: 29 title: Clean  Clear ESSENTIALS Dual Action Moisturizer, 4 Ounce, id: 34 title: Cetaphil Gentle Cleansing Bar, Antibacterial - 4.5 oz recommend next item
\tabularnewline 
\hline
Next Item & id: 6724 title: Head Shoulders Clinical Strength Dandruff Shampoo 14.2 Fl Oz (Pack of 2) (packaging may vary)
\tabularnewline 
\hline
\multicolumn{2}{l}{\textbf{Sports}}
\tabularnewline 
\hline
User Interaction History & Here is the visit history list of user: id: 18308 title: Rubbermaid  Shaker Bottle, 20-Ounce, Purple, id: 7317 title: GSI Outdoors Glacier Stainless Steel Plate, id: 17627 title: NOCO Genius GENM2 8 Amp 2-Bank Waterproof Smart On-Board Battery Charger, id: 385 title: Lodge Pro-Logic P12D3 Cast Iron Dutch Oven, Black, 7-Quart, id: 15 title: Lodge Original Finish Pro Grid/Iron Griddle recommend next item
\tabularnewline 
\hline
Next Item & id: 17944 title: Yoga Full Toe Socks (Various Colors), 2 Pairs Value Pack Set
\tabularnewline 
\hline
\multicolumn{2}{l}{\textbf{Toys}}
\tabularnewline 
\hline
User Interaction History & Here is the visit history list of user: id: 188 title: Little Tikes Cozy Coupe, id: 423 title: Music  Lights Sit 'n Spin Rockin' Tunes (colors vary), id: 381 title: Naturally Playful Kangaroo Climber, id: 211 title: Elmo's Rock  Roll Guitar recommend next item
\tabularnewline 
\hline
Next Item & id: 412 title: Turtle Sandbox
\tabularnewline 
\hline 
\end{tabular}
 \caption{Text Representations of Items Used in SREDR. We sample four cases from Yelp, Beauty, Sports, and Toys, to show  the verbalization results of user-item interaction history and items.}
 \label{tab:verbalization}
\end{table*}

==> table/lowhighfreq.tex <==
\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ l | c  |  c | c | c | c  }
\hline
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{\#Threshold}} & \multicolumn{2}{c|}{\textbf{Low Frequency}} & \multicolumn{2}{c}{\textbf{High Frequency}} \\ \cline{3-6}
& & \#Item   & \#Sample   & \#Item   & \#Sample \\
\hline
Beauty & 16 & 6365 & 13767 & 1613 & 8596  \\
Yelp & 19 & 10207 & 17756 & 2723 & 12743  \\
Sports & 16 & 10073 & 21831 & 2521 & 13767  \\
Toys & 15 & 5924 & 12718 & 1551 & 6694  \\
\hline
\end{tabular}}
\caption{Data Statistics with Different User Interacted Frequencies. We set the threshold according to the ratio of 8:2~\cite{ZhihongChen2020ESAMDD} to divide the label items in the test set into low-frequency items and high-frequency items. We split the testing datasets into two groups, low frequency and higher frequency, according to the user interacted frequency of items.}
\label{tab:freq}
\end{table}

==> table/suboverall.tex <==
% \begin{table}[t]
% \begin{center}
% \small
% \resizebox{0.49\textwidth}{!}{
% \begin{tabular}{l|c|   c  c  c   c  | c }
% \hline 
% \textbf{Datasets} & \textbf{Metrics} &  \textbf{GRU4Rec}  &  \textbf{NOVA}  & \textbf{ICAI-SR}  & \textbf{DIF-SR} &  \textbf{SREDR}\\ 
% \hline
% \multirow{4}{*}{Beauty} & Recall@10 & 0.0530 &  0.0887  &0.0879 & \uline{0.0908}  & \textbf{0.0935}  \\
% & Recall@20  & 0.0839  & 0.1237 & 0.1231 & \uline{0.1284} & \textbf{0.1441}  \\
% & NDCG@10  & 0.0266 & 0.0439 & 0.0439& \uline{\textbf{0.0446}} & 0.0445  \\
% & NDCG@20  &0.0344  & 0.0527 & 0.0528 & \uline{0.0541} & \textbf{0.0573}  \\
% \hline
% \multirow{4}{*}{Sports} & Recall@10   &0.0312 &0.0534 & 0.0527 & \uline{\textbf{0.0556}}  & 0.0545 \\
% & Recall@20 &0.0482 &0.0759 &0.0762 & \uline{0.0800}  & \textbf{0.0851} \\
% & NDCG@10  &0.0157 &0.0250 &0.0243 & \uline{0.0264}  & \textbf{0.0270}  \\
% & NDCG@20 &0.0200 &0.0307 & 0.0302 & \uline{0.0325}  & \textbf{0.0346}  \\
% \hline
% \multirow{4}{*}{Toys} & Recall@10  & 0.0370 &  0.0978  &0.0972 & \uline{0.1013} & \textbf{0.1056} \\
% & Recall@20  & 0.0588  & 0.1322 & 0.1303 & \uline{0.1382}  & \textbf{0.1594} \\
% & NDCG@10 & 0.0184 & 0.0480 & 0.0478  & \uline{0.0504} & \textbf{0.0508} \\
% & NDCG@20 &0.0239  & 0.0567 & 0.0561 & \uline{0.0597} & \textbf{0.0643} \\
% \hline
% \multirow{4}{*}{Yelp} & Recall@10  & 0.0361 &  0.0681  &0.0663  & \uline{0.0698} & \textbf{0.0733} \\
% & Recall@20 & 0.0592  & 0.0964 & 0.0940 & \uline{0.1003}  & \textbf{0.1150} \\
% & NDCG@10  & 0.0184 & 0.0412 & 0.0400 & \uline{\textbf{0.0419}}  & 0.0393  \\
% & NDCG@20 &0.0243  & 0.0483 & 0.0470 & \uline{0.0496} & \textbf{0.0498} \\
%  \hline

% \end{tabular}}
% \end{center}
% \caption{\label{tab:suboverall}Additional Compared Results. }

% \end{table}

\begin{table}[t]
\begin{center}
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|c|   c  c  c   | c }
\hline 
\textbf{Dataset} & \textbf{Metrics} &  \textbf{GRU4Rec}  &  \textbf{NOVA}  & \textbf{ICAI-SR}  &  \textbf{SREDR}\\ 
\hline
\multirow{4}{*}{Beauty} & Recall@10 & 0.0530 &  0.0887  &0.0879 & \textbf{0.1030}  \\
& Recall@20  & 0.0839  & 0.1237 & 0.1231 & \textbf{0.1550}  \\
& NDCG@10  & 0.0266 & 0.0439 & 0.0439 & \textbf{0.0517}  \\
& NDCG@20  &0.0344  & 0.0527 & 0.0528 & \textbf{0.0649}  \\
\hline
\multirow{4}{*}{Sports} & Recall@10   &0.0312 &0.0534 & 0.0527 & \textbf{0.0633} \\
& Recall@20 &0.0482 &0.0759 &0.0762 & \textbf{0.0964} \\
& NDCG@10  &0.0157 &0.0250 &0.0243 & \textbf{0.0338}  \\
& NDCG@20 &0.0200 &0.0307 & 0.0302 & \textbf{0.0421}  \\
\hline
\multirow{4}{*}{Toys} & Recall@10  & 0.0370 &  0.0978  &0.0972 & \textbf{0.1232} \\
& Recall@20  & 0.0588  & 0.1322 & 0.1303 & \textbf{0.1789} \\
& NDCG@10 & 0.0184 & 0.0480 & 0.0478  & \textbf{0.0640} \\
& NDCG@20 &0.0239  & 0.0567 & 0.0561 & \textbf{0.0780} \\
\hline
\multirow{4}{*}{Yelp} & Recall@10  & 0.0361 &  0.0681  &0.0663  & \textbf{0.0738} \\
& Recall@20 & 0.0592  & 0.0964 & 0.0940  & \textbf{0.1156} \\
& NDCG@10  & 0.0184 & \textbf{0.0412} & 0.0400 & 0.0397  \\
& NDCG@20 &0.0243  & 0.0483 & 0.0470 & \textbf{0.0502} \\
 \hline
\end{tabular}}
\end{center}
\caption{\label{tab:suboverall} Experimental Results of Additional Baseline Models. }

\end{table}

==> table/tokenstatistic.tex <==

\begin{table*}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ l | r r r | r r r | r r r | r r r }
\hline
\multirow{2}{*}{\textbf{Num}} & \multicolumn{3}{c}{\textbf{Beauty}} & \multicolumn{3}{c}{\textbf{Yelp}} & \multicolumn{3}{c}{\textbf{Sports}} & \multicolumn{3}{c}{\textbf{Toys}}  \\ \cline{2-13}
& Train   & Dev & Test & Train   & Dev & Test & Train   & Dev & Test & Train   & Dev & Test\\\hline
>256 & 37,857 & 4,634 & 5,693 & 44,035 & 3,158 & 3,507 & 34,374 & 5,267 & 6,533 & 21,663 & 2,173 & 2,577  \\
>512 & 19,185 & 1,472 & 1,663 & 16,017 & 842 & 911 & 11,728 & 1,165 & 1,335 & 9,384 & 607 & 661  \\
Mean & 276 & 221 & 252 & 164 & 132 & 147 & 172 & 172 & 198 & 183 & 151 & 173  \\
Mid & 129 & 142 & 173 & 92 & 87 & 102 & 100 & 125 & 152 & 93 & 106 & 128  \\
Mode & 40 & 95 & 135 & 25 & 55 & 71 & 34 & 89 & 118 & 31 & 76 & 100  \\
\hline
\end{tabular}}
\caption{Statistics of Text Tokens of User-Item Interaction Sequences.}
\label{tab:token}
\end{table*}

==> table/userid.tex <==
\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ l | c  |  c  | c  }
\hline
\multirow{2}{*}{\textbf{Settings}} & \multicolumn{1}{c|}{\textbf{Yelp}} & \multicolumn{1}{c|}{\textbf{Sports}} & \multicolumn{1}{c}{\textbf{Beauty}}\\ \cline{2-4}
& Recall@20   & Recall@20   & Recall@20 \\
\hline
T5-DPR & 0.0740& 0.0554 & 0.1082  \\
+ user id & 0.0419 & 0.0207 & 0.0557  \\
\hline
\end{tabular}}
\caption{Recommendation Performance of user identifier modeling.}
\label{tab:userid}
\end{table}
